WAccess -- A Web Accessibility Tool based on WCAG 2.2, 2.1 and 2.0 Guidelines

The vision of providing access to all web content equally for all users makes web accessibility a fundamental goal of today's internet. Web accessibility is the practice of removing barriers from websites that could hinder functionality for users with various disabilities. Web accessibility is measured against the accessibility guidelines such as WCAG, GIGW, and so on. WCAG 2.2 is the latest set of guidelines for web accessibility that helps in making websites accessible. The web accessibility tools available in the World Wide Web Consortium (W3C), only conform up to WCAG 2.1 guidelines, while no tools exist for the latest set of guidelines. Despite the availability of several tools to check the conformity of websites with WCAG 2.1 guidelines, there is a scarcity of tools that are both open source and scalable. To support automated accessibility evaluation of numerous websites against WCAG 2.2, 2.1, and 2.0 we present a tool, WAccess. WAccess highlights violations of 13 guidelines from WCAG 2.0, 9 guidelines from WCAG 2.1, and 7 guidelines from WCAG 2.2 of a specific web page on the web console and suggests the fix for violations while specifying violating code snippet simultaneously. We evaluated WAccess against 2227 government websites of India and observed a total of about 6.1 million violations.

==> Sections/commented-tables.tex <==
% \begin{table}
%       \begin{tabular}{|l|l|l|l|}
% \hline
% Guidelines                & ID     & Description                 & Level \\ \hline
% \multirow{7}{*}{WCAG 2.2} & 3.3.7  & Accessible Authentication   & A     \\ \cline{2-4} 
%                           & 2.5.7  & Dragging Movements          & AA    \\ \cline{2-4} 
%                           & 2.4.11 & Focus Appearance (Minimum)  & AA    \\ \cline{2-4} 
%                           & 2.4.12 & Focus Appearance (Enhanced) & AAA   \\ \cline{2-4} 
%                           & 2.4.13 & Page Break Navigation       & A     \\ \cline{2-4} 
%                           & 2.5.8  & Target Size (Minimum)       & AA    \\ \cline{2-4} 
%                           & 3.2.7  & Visible Controls            & A     \\ \hline
% \multirow{9}{*}{WCAG 2.1} & 1.3.5  & Identify Input Purpose      & AA    \\ \cline{2-4} 
%                           & 1.3.6  & Identify Purpose            & AAA   \\ \cline{2-4} 
%                           & 1.4.11 & Non-Text Contrast           & AA    \\ \cline{2-4} 
%                           & 1.4.13 & Content on Hover or Focus   & AA    \\ \cline{2-4} 
%                           & 2.1.4  & Character Key Shortcuts     & A     \\ \cline{2-4} 
%                           & 2.3.3  & Animation from Interactions & AAA   \\ \cline{2-4} 
%                           & 2.5.3  & Label in Name               & A     \\ \cline{2-4} 
%                           & 2.5.5  & Target Size                 & AAA   \\ \cline{2-4} 
%                           & 4.1.3  & Status Messages             & AA    \\ \hline
% \end{tabular}
%     \caption{Accessibility Guidelines considered for developing \textit{WAccess}}
%     \label{tab:table2}
% \end{table}


% \begin{table}
%         \begin{tabular}{|l|l|l|l|}
%             \hline
%             \textbf{Guidelines} & \textbf{ID} &  \textbf{Description} & \textbf{Level} \\\hline
% \multirow{}{}{WCAG 2.2} &
% \multicolumn{1}{|l|}{3.3.7} & \multicolumn{1}{|l|}{Accessible Authentication} & \multicolumn{1}{|l|}{A}\\\cline{2-4}
%                                  & 
% \multicolumn{1}{|l|}{2.5.7} & \multicolumn{1}{|l|}{Dragging Movements} & \multicolumn{1}{|l|}{AA}
                           
                                 

%             \\\hline
%             \multirow{}{}{WCAG 2.1} & \multicolumn{1}{|l|}{1.3.5} & \multicolumn{1}{|l|}{Identify Input Purpose} &
%             \multicolumn{1}{|l|}{AA}
%             \\\cline{2-4}
%                                  & \multicolumn{1}{|l|}{1.3.6} & \multicolumn{1}{|l|}{Identify Purpose} & \multicolumn{1}{|l|}{AAA}\\\cline{2-4}
%                                  & \multicolumn{1}{|l|}{1.4.11} & \multicolumn{1}{|l|}{Non-Text Contrast}& \multicolumn{1}{|l|}{AA} \\\cline{2-4}
%                                  & \multicolumn{1}{|l|}{1.4.13} & \multicolumn{1}{|l|}{Content on Hover or Focus}& \multicolumn{1}{|l|}{AA}
                    
%                     \\\cline{2-4}
%                                  & \multicolumn{1}{|l|}{2.1.4} & \multicolumn{1}{|l|}{Character Key Shortcuts}& \multicolumn{1}{|l|}{A}
%                                   \\\cline{2-4}
%                                  & \multicolumn{1}{|l|}{2.3.3} & \multicolumn{1}{|l|}{Animation from Interactions}& \multicolumn{1}{|l|}{AAA}
%                       \\\cline{2-4}
%                                  & \multicolumn{1}{|l|}{2.5.3} & \multicolumn{1}{|l|}{Label in Name}& \multicolumn{1}{|l|}{A}
%                       \\\cline{2-4}
%                                  & \multicolumn{1}{|l|}{2.5.5} & \multicolumn{1}{|l|}{Target Size}& \multicolumn{1}{|l|}{AAA}
%                       \\\cline{2-4}
%                                  & \multicolumn{1}{|l|}{4.1.3} & \multicolumn{1}{|l|}{Status Messages}& \multicolumn{1}{|l|}{AA}
%                                  \\\hline
            
%         \end{tabular}
%     \caption{Accessibility Guidelines considered for developing \textit{WAccess}}
%     \label{tab:table2}
% \end{table}

